On the Origin of the Strong Optical Variability of Emission-line Galaxies

Emission-line galaxies (ELGs) are crucial in understanding the formation and evolution of galaxies, while little is known about their variability. Here we report the study on the optical variability of a sample of ELGs selected in the COSMOS field, which has narrow-band observations in two epochs separated by $\gtrsim$ 12 years. This sample was observed with Suprime-Cam (SC) and Hyper Suprime-Cam (HSC) on the $Subaru$ telescope in NB816 and $i'/i$ bands, respectively. After carefully removing the wing effect of a narrow-band filter, we check the optical variability in a sample of 181 spectroscopically confirmed ELGs. We find that 0 (0/68) Ha emitters, 11.9% (5/42) [OIII] emitters, and 0 (0/71) [OII] emitters show significant variability ($|\Delta m_{NB}| \geq 3\,\sigma_{\Delta m_{NB,AGN}} = 0.20\, mag$) in the two-epoch narrow-band observations. We investigate the presence of active galactic nucleus (AGN) in this variable ELG (var-ELG) sample with three methods, including X-ray luminosity, mid-infrared activity, and radio-excess. We find zero bright AGN in this var-ELG sample, but cannot rule out the contribution from faint AGN. We find that SNe could also dominate the variability of the var-ELG sample. The merger morphology shown in the HST/F814W images of all the var-ELG sample is in agreement with the enhancement of star formation, i.e., the SNe activity.

==> table/table_AGN_in_variable_ELGs.tex <==
\begin{table*}
    \centering
	\caption{Identification of AGN in variable ELGs}
	\label{tab:variable_ELGs}
	\setlength{\tabcolsep}{0.5mm}{
    \begin{tabular}{cccccccc} \hline\hline
    \multirow{2}{*}{Line} & \multirow{2}{*}{number} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}percent in ELGs\end{tabular}}  & \multicolumn{5}{c}{AGN in variable ELGs} \\ 
     \cline{4-8} & & & 
     \begin{tabular}[c]{@{}c@{}}X-ray\\ selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIR\\
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}Radio\\ 
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}total\\ 
    number\end{tabular} & \begin{tabular}[c]{@{}c@{}}total\\ 
    percent\end{tabular} \\ 
    \hline
    % H$\alpha$           & 2   &2.8\%    & 0    & 0   &0   & 0  & 0   \\
    % {[}O{\sc iii}{]}    & 7   &11.5\%   & 0    & 0   &0   & 0  & 0   \\
    % {[}O{\sc ii}{]}     & 6   &4.4\%    & 0    & 0   &0   & 0  & 0   \\
     H$\alpha$          & 2    &2.5\%    & 0    & 0   &0   & 0  & 0   \\
    {[}O{\sc iii}{]}    & 3    &4.3\%    & 0    & 0   &0   & 0  & 0   \\
    {[}O{\sc ii}{]}     & 9   &6.1\%    & 0    & 0   &0   & 0  & 0   \\
    \hline\hline
    \end{tabular}}
\end{table*}


==> table/table_AGN_var-ELG.tex <==
\addtocounter{table}{-1}
\begin{table*}
    \centering
    % \footnotesize
    \caption{Physical parameters of variable ELGs (continued)}
    \label{tab:AGN_selection}
    % \begin{threeparttable}
    \setlength{\tabcolsep}{0.4cm}{
    \begin{tabular}{lccccccccc} \hline \hline
    \multirow{2}{*}{Var-ID} 
    & \multirow{2}{*}{line} 
    & X-ray 
    & MIR  
    &  radio 
    & \multirow{2}{*}{AGN?} 
    & \multirow{2}{*}{spec-z}  
    & $\rm SFR_{HSC}$ 
    & $\rm SFR_{SC}$ 
    \\
    &  & AGN?  & AGN?  & AGN? &  &  & ($\rm M_{\odot}\cdot year^{-1}$)& ($\rm M_{\odot}\cdot year^{-1}$)  \\
    \hline
    % var-ELG1  & H$\alpha$   & 0  & 0  & 0 & 0 & 0.236 & 0.18$^a$/0.12$^b$  & 0.10$^a$/0.07$^b$  \\
    % var-ELG2  & H$\alpha$   & 0  & 0   & 0 & 0  & 0.237 & 0.85$^a$/0.57$^b$  & 0.49$^a$/0.33$^b$  \\
    % var-ELG3  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.620 & 6.15$^c$  & 3.68$^c$  \\
    % var-ELG4  & [O{\sc iii}] & 0  & 0  & 0 & 0  & 0.620 & 11.59$^c$ & 7.34$^c$  \\
    % var-ELG5  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.622 & 1.23$^c$  & 0.79$^c$  \\
    % var-ELG6  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.630 & 0.32$^c$  & 0.52$^c$  \\
    % var-ELG7  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.636 & 0.76$^c$  & 1.69$^c$  \\
    % var-ELG8  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.639 & 0.22$^c$  & 0.44$^c$  \\
    % var-ELG9  & [O{\sc iii}] & 0  & 0  & 0 & 0  & 0.639 & 3.13$^c$  & 5.16$^c$  \\
    % var-ELG10 & [O{\sc ii}]  & 0 & 0  & 0 & 0  & 1.175 & 40.62$^d$ & 26.19$^d$ \\
    % var-ELG11 & [O{\sc ii}]  & 0 & 0  & 0 & 0  & 1.175 & 31.20$^d$ & 18.71$^d$ \\
    % var-ELG12 & [O{\sc ii}]  & 0  & 0  & 0 & 0  & 1.176 & 25.07$^d$ & 15.27$^d$ \\
    % var-ELG13 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.181 & 1.24$^d$  & 2.08$^d$  \\
    % var-ELG14 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.197 & 1.33$^d$  & 2.57$^d$  \\
    % var-ELG15 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.198 & 1.14$^d$  & 2.66$^d$  \\ \hline \hline
    % % \multicolumn{9}{l}{\begin{tabular}[l]{p{12cm}} $^a$ follows Kennicutt 1998; $^b$ follows Kennicutt \& Evans, 2012; $^c$ follows Zhuang \& Ho, 2019; $^d$ follows Villa-Vélez et al. 2021 (in prepare). Column 1 and 2 are same as table.~\ref{tab:photometry}; Column 3-4: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite and dashes means uncovered; Column 5: radio selected AGN from~\citet{Delvecchio2017}; Column 6: total count of AGN via above methods; Column 7: spectroscopic redshift; Column 8-9: SFR calculated using emission-line indicator measured with HSC and SC as described in section~\ref{sec:SFR}.\end{tabular}} \\
        
   var-ELG1  & H$\alpha$   & 0 & 0 & 0 & 0 & 0.236 & 0.19$^a$/0.13$^b$  & 0.10$^a$/0.07$^b$  \\
    var-ELG2  & H$\alpha$   & 0 & 0 & 0 & 0 & 0.237 & 0.88$^a$/0.59$^b$  & 0.49$^a$/0.33$^b$  \\
    var-ELG3  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.62  & 6.32$^c$  & 3.69$^c$  \\
    var-ELG4  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.62  & 11.87$^c$ & 7.37$^c$  \\
    var-ELG5  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.636 & 0.79$^c$  & 1.70$^c$  \\
    var-ELG6  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 21.26$^d$ & 12.61$^d$ \\
    var-ELG7  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 19.25$^d$ & 12.50$^d$ \\
    var-ELG8  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 41.77$^d$ & 26.16$^d$ \\
    var-ELG9  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 32.36$^d$ & 19.02$^d$ \\
    var-ELG10 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.176 & 26.03$^d$ & 15.36$^d$ \\
    var-ELG11 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.177 & 2.35$^d$  & 1.45$^d$  \\
    var-ELG12 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.187 & 0.96$^d$  & 1.46$^d$  \\
    var-ELG13 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.197 & 1.24$^d$  & 2.51$^d$  \\
    var-ELG14 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.198 & 2.56$^d$  & 4.22$^d$  \\ \hline \hline
    \end{tabular}}
    \begin{tablenotes}
    \item Column 1 and 2 are the same to table.~\ref{tab:photometry}; Column 3-4: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite; Column 5: radio selected AGN from~\citet{Delvecchio2017}; Column 6: total number of AGN via above three methods; Column 7: spectroscopic redshift; Column 8-9: SFRs of variable ELGs calculated by emission-line indicator in HSC-phase and SC-phase, as described in section~\ref{sec:SFR}. $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; $^c$ follows~\citet{Zhuang2019}; $^d$ follows~\citet{Villa2021}.
    \end{tablenotes}
    % \end{threeparttable}
\end{table*}

==> variable ELG/latex_morphology.tex <==
\begin{figure*}
% \subfigure{ 
\centering
% \includegraphics[width=0.8\linewidth]{morphology/1}
% \includegraphics[width=0.8\linewidth]{morphology/2}
% \includegraphics[width=0.8\linewidth]{morphology/3}
% \includegraphics[width=0.8\linewidth]{morphology/4}
% \includegraphics[width=0.8\linewidth]{morphology/5}
% \includegraphics[width=0.8\linewidth]{morphology/6}
% \includegraphics[width=0.8\linewidth]{morphology/7}
% \includegraphics[width=0.8\linewidth]{morphology/8}
% \includegraphics[width=0.8\linewidth]{morphology/9}
% \includegraphics[width=0.8\linewidth]{morphology/10}
% \includegraphics[width=0.8\linewidth]{morphology/11}
% \includegraphics[width=0.8\linewidth]{morphology/12}
\includegraphics[width=0.7\linewidth]{morphology/var_ELG.png}
\caption{Image cutouts of \revise{5} var-ELGs. All stamps are in a size of 5\arcsec $\times$ 5\arcsec. Column 1-2:   NB816 and $i'$-band with SC; Column 3-4: NB816 and i-band with HSC; Column 5:  HST/F814W band. The circles with white dashed lines have 3\arcsec\ diameters.}
% \caption{Morphologies of variable ELGs. Column 1-2:  5\arcsec $\times$ 5\arcsec NB816 and i-band images of variable ELGs with HSC; Column 3-4: 5\arcsec $\times$ 5\arcsec NB816 and i$^+$-band images with SC, respectively; Column 5: 5\arcsec $\times$ 5\arcsec HST images in F814W band; Column 6-8: 15\arcsec $\times$ 15\arcsec Soft (0.5 - 2.0 kev), full (0.5 - 7.0 kev) and hard (2.0 - 7.0 kev) X-ray images observed by Chandra and the green regions are of size of 5\arcsec $\times$ 5\arcsec.}

\label{fig:morpholigy1} 
\end{figure*}

% \addtocounter{figure}{-1}
% \begin{figure*}
% \centering
% \includegraphics[width=0.8\linewidth]{morphology/var_ELG2.png}
%  \caption{Morphology of variable ELGs (continued).}
% \end{figure*}



% \addtocounter{figure}{-1}
% \begin{figure*}
% \centering
% \includegraphics[width=0.8\linewidth]{morphology/13}
% \includegraphics[width=0.8\linewidth]{morphology/14}
% \includegraphics[width=0.8\linewidth]{morphology/15}
% \includegraphics[width=0.8\linewidth]{morphology/16}
% \includegraphics[width=0.8\linewidth]{morphology/17}
% \includegraphics[width=0.8\linewidth]{morphology/18}
% \includegraphics[width=0.8\linewidth]{morphology/19}
% \includegraphics[width=0.8\linewidth]{morphology/20}
% \includegraphics[width=0.8\linewidth]{morphology/21}
% \includegraphics[width=0.8\linewidth]{morphology/22}
% \includegraphics[width=0.8\linewidth]{morphology/23}
% \includegraphics[width=0.8\linewidth]{morphology/24}
%  \caption{Morphology of variable ELGs (continued).}
% % }
% \end{figure*}

% \addtocounter{figure}{-1}
% \begin{figure*}
% \centering
% \includegraphics[width=0.8\linewidth]{morphology/25}
% \includegraphics[width=0.8\linewidth]{morphology/26}
% \includegraphics[width=0.8\linewidth]{morphology/27}
% \caption{Morphology of variable ELGs (continued).}
% % }
% \end{figure*}

==> variable ELG/table/observation_date.tex <==
\begin{table}[]
\centering
    % \footnotesize
	\caption{Observation Dates of i'/i and NB816 bands with SC and HSC}
	\label{tab:observing_date}
	\setlength{\tabcolsep}{0.2cm}{
\begin{tabular}{c|cc} \hline \hline
filter & SC  & HSC \\ \hline
i'/i   & \begin{tabular}[c]{@{}c@{}} Feb. 2004, \\  Jan. 2004\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Jan. 2020,\\  May. 2019,\\  Apr. 2017,\\  Mar. 2017,\\  Feb. 2017,\\  Jan. 2017,\\  Dec. 2016,\\  Nov. 2016,\\  Feb. 2016\end{tabular} \\ \hline
NB816  & \begin{tabular}[c]{@{}c@{}} Apr. 2005,\\  Mar. 2005,\\  Feb. 2005,\\  Apr. 2004\end{tabular} & \begin{tabular}[c]{@{}c@{}} Mar. 2019,\\  Feb. 2019,\\  Feb. 2016\end{tabular}    \\ \hline \hline                                                                                                            
\end{tabular}
}
\end{table}

==> variable ELG/table/table_AGN_in_ELGs.tex <==
\begin{table*}
    \centering
    % \begin{center}
    % \footnotesize
	\caption{Statistics of the ELG sample}
	\label{tab:ELGs}
	\setlength{\tabcolsep}{0.03cm}{
    % \begin{tabular}{cccccccccc} \hline\hline
    \begin{tabular}{ccccccccc} \hline\hline
    \multirow{3}{*}{Line} &
    \multirow{3}{*}{Spec-{\it z} range} &
    \multirow{3}{*}{\#(ELGs)} &
        \multirow{3}{*}{\#(var-ELGs)} &
    % \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}number\\ in {\it ELG sub-sample} \end{tabular}} &
    \multicolumn{5}{c}{\#(AGN) in ELGs} \\ 
     \cline{5-9} &  &  & & \begin{tabular}[c]{@{}c@{}}X-ray\\ 
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIR\\ 
    % selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}SED\\ 
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}Radio\\
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}\revise{BPT}\\
    \revise{selected}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}\#(AGN)\\ 
    \end{tabular} 
    % & \begin{tabular}[c]{@{}c@{}}X-ray AGN\\ 
    % fraction$^a$\end{tabular} & \begin{tabular}[c]{@{}c@{}}total\\ 
    % fraction\end{tabular} 
    \\ 
    \hline
    % H$\alpha$           & 0.236 - 0.251     & 71    &   & 1   & 3   &0   & 3   & 0              & 4.2\%   \\
    % {[}O{\sc iii}{]}    & 0.620 - 0.640     & 61    &   & 1   & 1   &1   & 1   & 1.6\%(1/61)    & 1.6\%   \\
    % {[}O{\sc ii}{]}     & 1.175 - 1.201     & 136   &   & 4   & 18  &1   & 20  & 2.9\% (4/136)  & 14.7\%  \\
    H$\alpha$           & 0.238 - 0.250     &  68 & 0  &  1 $(0^a)$ & 0   &0   & \revise{2/42}$^e$ & \revise{3}     \\
    %  & & & & \multicolumn{5}{c}{$log(\nu L_{\nu,limit})$ (z$\sim$0.25)} \\ 
    %  \cline{5-9} 
    & & & & [41.5]$^b$ & [41.1,41.3,42.0,42.0]$^c$ & [34.0,35.1]$^d$ &  & \\
    {[}O{\sc iii}{]}    & 0.623 - 0.639     &  \revise{42} & \revise{5} &  0         & 0   &0   & \revise{--} & 0     \\
    % & & & & \multicolumn{5}{c}{$log(\nu L_{\nu,limit})$ (z$\sim$0.62)} \\ 
    %  \cline{5-9} 
    & & & & [42.2]$^b$ & [42.1,42.3,43.0,42.9]$^c$ & [34.9,36.0]$^d$ &  & \\
    {[}O{\sc ii}{]}     & 1.181 - 1.202     &  \revise{71} & \revise{0} &  \revise{5 $(5^a)$} & 11  &\revise{2}   & \revise{--} & \revise{14}    \\
    % & & & & \multicolumn{5}{c}{$log(\nu L_{\nu,limit})$ (z$\sim$1.19)} \\ 
    %  \cline{5-9} 
    & & & & [42.9]$^b$ & [42.8,42.9,43.7,43.6]$^c$ & [35.6,36.7]$^d$ &  & \\
    \hline
    % \multicolumn{9}{l}{$^a$ Selection criterion of X-ray bright AGN: $\rm L_X \geqq 10^{43}\ erg\cdot s^{-1}$} \\
    % \multicolumn{9}{l}{$^b$ The detected luminosity limit for each method in unit of $erg\,s^{-1}$. For the X-ray method, we present the luminosity in the full band. For MIR method, } \\
    \end{tabular}
    }
    \begin{tablenotes}
    \footnotesize
    \item $^a$ Selection criterion of X-ray bright AGN: $\rm L_X \geqq 10^{43}\ erg\cdot s^{-1}$. 
    \item $^b$ \revise{The 5-$\sigma$ luminosity (log$L$) detection limit in the X-ray 0.5-10 keV band. }
    \item $^c$ \revise{The 5-$\sigma$ luminosity (log$\nu L_\nu$) detection limits in the 3.6, 4.5, 5.8, and 8.0 $\mu m$ bands. }
    \item $^d$ \revise{The 5-$\sigma$ luminosity (log$\nu L_\nu$) detection limits in the 3 and 1.4 GHz bands.}
    \item $^e$ \revise{Only 42 out of 68 H$\alpha$ emitters were covered by the $z$COSMOS spectroscopic survey, and the BPT diagnostic was applied to this sub-sample.}
    \end{tablenotes}
    % \end{center}
    % \tablecomments{$^a$ AGN-selected criterion of $\rm L_X \geqq 10^{43} erg\cdot s^{-1}$}
\end{table*}


==> variable ELG/table/table_AGN_in_variable_ELGs.tex <==
\begin{table*}
    \centering
	\caption{Identification of AGN in variable ELGs}
	\label{tab:variable_ELGs}
	\setlength{\tabcolsep}{0.5mm}{
    \begin{tabular}{cccccccc} \hline\hline
    \multirow{2}{*}{Line} & \multirow{2}{*}{number} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}percent in ELGs\end{tabular}}  & \multicolumn{5}{c}{AGN in variable ELGs} \\ 
     \cline{4-8} & & & 
     \begin{tabular}[c]{@{}c@{}}X-ray\\ selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIR\\
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}Radio\\ 
    selected\end{tabular} & \begin{tabular}[c]{@{}c@{}}total\\ 
    number\end{tabular} & \begin{tabular}[c]{@{}c@{}}total\\ 
    percent\end{tabular} \\ 
    \hline
    % H$\alpha$           & 2   &2.8\%    & 0    & 0   &0   & 0  & 0   \\
    % {[}O{\sc iii}{]}    & 7   &11.5\%   & 0    & 0   &0   & 0  & 0   \\
    % {[}O{\sc ii}{]}     & 6   &4.4\%    & 0    & 0   &0   & 0  & 0   \\
     H$\alpha$          & 2    &2.5\%    & 0    & 0   &0   & 0  & 0   \\
    {[}O{\sc iii}{]}    & 3    &4.3\%    & 0    & 0   &0   & 0  & 0   \\
    {[}O{\sc ii}{]}     & 9   &6.1\%    & 0    & 0   &0   & 0  & 0   \\
    \hline\hline
    \end{tabular}}
\end{table*}


==> variable ELG/table/table_AGN_var-ELG.tex <==
\addtocounter{table}{-1}
\begin{table*}
    \centering
    % \footnotesize
    \caption{Physical parameters of variable ELGs (continued)}
    \label{tab:AGN_selection}
    % \begin{threeparttable}
    \setlength{\tabcolsep}{0.4cm}{
    \begin{tabular}{lccccccccc} \hline \hline
    \multirow{2}{*}{Var-ID} 
    & \multirow{2}{*}{line} 
    & X-ray 
    & MIR  
    &  radio 
    & \multirow{2}{*}{AGN?} 
    & \multirow{2}{*}{spec-z}  
    & $\rm SFR_{HSC}$ 
    & $\rm SFR_{SC}$ 
    \\
    &  & AGN?  & AGN?  & AGN? &  &  & ($\rm M_{\odot}\cdot year^{-1}$)& ($\rm M_{\odot}\cdot year^{-1}$)  \\
    \hline
    % var-ELG1  & H$\alpha$   & 0  & 0  & 0 & 0 & 0.236 & 0.18$^a$/0.12$^b$  & 0.10$^a$/0.07$^b$  \\
    % var-ELG2  & H$\alpha$   & 0  & 0   & 0 & 0  & 0.237 & 0.85$^a$/0.57$^b$  & 0.49$^a$/0.33$^b$  \\
    % var-ELG3  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.620 & 6.15$^c$  & 3.68$^c$  \\
    % var-ELG4  & [O{\sc iii}] & 0  & 0  & 0 & 0  & 0.620 & 11.59$^c$ & 7.34$^c$  \\
    % var-ELG5  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.622 & 1.23$^c$  & 0.79$^c$  \\
    % var-ELG6  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.630 & 0.32$^c$  & 0.52$^c$  \\
    % var-ELG7  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.636 & 0.76$^c$  & 1.69$^c$  \\
    % var-ELG8  & [O{\sc iii}] & 0  & 0  & 0 & 0 & 0.639 & 0.22$^c$  & 0.44$^c$  \\
    % var-ELG9  & [O{\sc iii}] & 0  & 0  & 0 & 0  & 0.639 & 3.13$^c$  & 5.16$^c$  \\
    % var-ELG10 & [O{\sc ii}]  & 0 & 0  & 0 & 0  & 1.175 & 40.62$^d$ & 26.19$^d$ \\
    % var-ELG11 & [O{\sc ii}]  & 0 & 0  & 0 & 0  & 1.175 & 31.20$^d$ & 18.71$^d$ \\
    % var-ELG12 & [O{\sc ii}]  & 0  & 0  & 0 & 0  & 1.176 & 25.07$^d$ & 15.27$^d$ \\
    % var-ELG13 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.181 & 1.24$^d$  & 2.08$^d$  \\
    % var-ELG14 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.197 & 1.33$^d$  & 2.57$^d$  \\
    % var-ELG15 & [O{\sc ii}]  & 0  & 0  & 0 & 0 & 1.198 & 1.14$^d$  & 2.66$^d$  \\ \hline \hline
    % % \multicolumn{9}{l}{\begin{tabular}[l]{p{12cm}} $^a$ follows Kennicutt 1998; $^b$ follows Kennicutt \& Evans, 2012; $^c$ follows Zhuang \& Ho, 2019; $^d$ follows Villa-Vélez et al. 2021 (in prepare). Column 1 and 2 are same as table.~\ref{tab:photometry}; Column 3-4: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite and dashes means uncovered; Column 5: radio selected AGN from~\citet{Delvecchio2017}; Column 6: total count of AGN via above methods; Column 7: spectroscopic redshift; Column 8-9: SFR calculated using emission-line indicator measured with HSC and SC as described in section~\ref{sec:SFR}.\end{tabular}} \\
        
   var-ELG1  & H$\alpha$   & 0 & 0 & 0 & 0 & 0.236 & 0.19$^a$/0.13$^b$  & 0.10$^a$/0.07$^b$  \\
    var-ELG2  & H$\alpha$   & 0 & 0 & 0 & 0 & 0.237 & 0.88$^a$/0.59$^b$  & 0.49$^a$/0.33$^b$  \\
    var-ELG3  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.62  & 6.32$^c$  & 3.69$^c$  \\
    var-ELG4  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.62  & 11.87$^c$ & 7.37$^c$  \\
    var-ELG5  & [O{\sc iii}] & 0 & 0 & 0 & 0 & 0.636 & 0.79$^c$  & 1.70$^c$  \\
    var-ELG6  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 21.26$^d$ & 12.61$^d$ \\
    var-ELG7  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 19.25$^d$ & 12.50$^d$ \\
    var-ELG8  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 41.77$^d$ & 26.16$^d$ \\
    var-ELG9  & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.175 & 32.36$^d$ & 19.02$^d$ \\
    var-ELG10 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.176 & 26.03$^d$ & 15.36$^d$ \\
    var-ELG11 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.177 & 2.35$^d$  & 1.45$^d$  \\
    var-ELG12 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.187 & 0.96$^d$  & 1.46$^d$  \\
    var-ELG13 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.197 & 1.24$^d$  & 2.51$^d$  \\
    var-ELG14 & [O{\sc ii}]  & 0 & 0 & 0 & 0 & 1.198 & 2.56$^d$  & 4.22$^d$  \\ \hline \hline
    \end{tabular}}
    \begin{tablenotes}
    \item Column 1 and 2 are the same to table.~\ref{tab:photometry}; Column 3-4: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite; Column 5: radio selected AGN from~\citet{Delvecchio2017}; Column 6: total number of AGN via above three methods; Column 7: spectroscopic redshift; Column 8-9: SFRs of variable ELGs calculated by emission-line indicator in HSC-phase and SC-phase, as described in section~\ref{sec:SFR}. $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; $^c$ follows~\citet{Zhuang2019}; $^d$ follows~\citet{Villa2021}.
    \end{tablenotes}
    % \end{threeparttable}
\end{table*}

==> variable ELG/table/table_photometry_of_variable_ELGs.tex <==
% \begin{table*}
%     \centering
%     % \footnotesize
%     \caption{Physical parameters of variable ELGs}
%     \label{tab:photometry}
%     % \begin{threeparttable}
%     \setlength{\tabcolsep}{1.5mm}{
%     % \resizebox{\textwidth}{30mm}{
%     \begin{tabular}{lccccccccc} \hline \hline
%     \multirow{2}{*}{Var-ID}
%     & \multirow{2}{*}{line}
%     & \multirow{2}{*}{ra} 
%     & \multirow{2}{*}{dec} 
%     & corrected HSC 
%     & HSC i 
%     & corrected SC 
%     & SC i  
%     & variation
%     % & \multicolumn{1}{c}{\multirow{2}{*}{redshift}} 
%     \\
%       &  &  &  & NB816 (mag) & (mag)  & NB816 (mag)  & (mag) & (mag)  
%     %   & 
%     \\ \hline
%     % 
%     % var-ELG1  & H$\alpha$   & 150.144366 & 2.228847 & 22.626$\pm$0.023 & 24.004$\pm$0.010 & 23.268$\pm$0.063 & 23.922$\pm$0.055 & -0.643$\pm$0.067 \\
%     % var-ELG2  & H$\alpha$   & 150.130035 & 2.215896 & 23.323$\pm$0.049 & 24.521$\pm$0.016 & 24.412$\pm$0.141 & 24.543$\pm$0.069 & -1.089$\pm$0.149 \\
%     % var-ELG3  & H$\alpha$   & 150.329992 & 2.671968 & 21.707$\pm$0.011 & 22.986$\pm$0.004 & 22.350$\pm$0.032 & 22.982$\pm$0.031 & -0.642$\pm$0.034 \\
%     % var-ELG4  & H$\alpha$   & 149.955237 & 2.607382 & 20.975$\pm$0.005 & 22.264$\pm$0.002 & 21.589$\pm$0.021 & 22.238$\pm$0.021 & -0.614$\pm$0.021 \\
%     % var-ELG5  & [O{\sc iii}] & 150.161848 & 2.022773 & 20.360$\pm$0.004 & 21.912$\pm$0.002 & 20.879$\pm$0.014 & 21.901$\pm$0.018 & -0.519$\pm$0.015 \\
%     % var-ELG6  & [O{\sc iii}] & 150.172093 & 2.068536 & 21.045$\pm$0.006 & 22.532$\pm$0.003 & 21.628$\pm$0.021 & 22.532$\pm$0.024 & -0.583$\pm$0.022 \\
%     % var-ELG7  & [O{\sc iii}] & 149.575281 & 2.311057 & 21.979$\pm$0.016 & 23.240$\pm$0.005 & 22.549$\pm$0.036 & 23.282$\pm$0.037 & -0.569$\pm$0.039 \\
%     % var-ELG8  & [O{\sc iii}] & 150.058745 & 2.331445 & 24.446$\pm$0.070 & 24.958$\pm$0.021 & 23.898$\pm$0.079 & 25.062$\pm$0.113 & 0.548$\pm$0.105  \\
%     % var-ELG9  & [O{\sc iii}] & 150.067333 & 2.473629 & 23.364$\pm$0.028 & 23.596$\pm$0.007 & 22.539$\pm$0.039 & 23.632$\pm$0.042 & 0.826$\pm$0.048  \\
%     % var-ELG10 & [O{\sc iii}] & 150.246630 & 2.155733 & 22.438$\pm$0.014 & 23.180$\pm$0.005 & 21.995$\pm$0.033 & 23.167$\pm$0.033 & 0.443$\pm$0.036  \\
%     % var-ELG11 & [O{\sc iii}] & 150.112667 & 2.537806 & 24.681$\pm$0.117 & 25.691$\pm$0.048 & 24.026$\pm$0.163 & 25.636$\pm$0.149 & 0.655$\pm$0.201  \\
%     % var-ELG12 & [O{\sc iii}] & 150.036836 & 2.681063 & 21.847$\pm$0.008 & 22.729$\pm$0.003 & 21.398$\pm$0.025 & 22.717$\pm$0.027 & 0.449$\pm$0.026  \\
%     % var-ELG13 & [O{\sc ii}]  & 150.315644 & 1.811455 & 21.852$\pm$0.013 & 23.040$\pm$0.004 & 22.435$\pm$0.033 & 23.108$\pm$0.032 & -0.583$\pm$0.036 \\
%     % var-ELG14 & [O{\sc ii}]  & 150.356427 & 2.551102 & 21.647$\pm$0.010 & 23.172$\pm$0.003 & 22.305$\pm$0.030 & 23.070$\pm$0.032 & -0.658$\pm$0.032 \\
%     % var-ELG15 & [O{\sc ii}]  & 149.778471 & 2.762363 & 21.769$\pm$0.013 & 23.088$\pm$0.005 & 22.239$\pm$0.030 & 23.091$\pm$0.034 & -0.470$\pm$0.033 \\
%     % var-ELG16 & [O{\sc ii}]  & 150.200091 & 2.018675 & 20.974$\pm$0.006 & 22.178$\pm$0.002 & 21.507$\pm$0.020 & 22.195$\pm$0.020 & -0.533$\pm$0.020 \\
%     % var-ELG17 & [O{\sc ii}]  & 150.144209 & 2.750572 & 20.928$\pm$0.006 & 22.723$\pm$0.003 & 21.428$\pm$0.020 & 22.694$\pm$0.027 & -0.500$\pm$0.020 \\
%     % var-ELG18 & [O{\sc ii}]  & 149.543684 & 2.553159 & 21.205$\pm$0.007 & 22.632$\pm$0.003 & 21.783$\pm$0.023 & 22.645$\pm$0.026 & -0.578$\pm$0.024 \\
%     % var-ELG19 & [O{\sc ii}]  & 149.941102 & 1.963592 & 21.661$\pm$0.010 & 22.995$\pm$0.004 & 22.227$\pm$0.029 & 23.005$\pm$0.031 & -0.566$\pm$0.030 \\
%     % var-ELG20 & [O{\sc ii}]  & 150.027007 & 2.116376 & 21.444$\pm$0.007 & 22.789$\pm$0.003 & 22.012$\pm$0.025 & 22.806$\pm$0.028 & -0.568$\pm$0.026 \\
%     % var-ELG21 & [O{\sc ii}]  & 150.521367 & 2.533642 & 21.542$\pm$0.009 & 22.610$\pm$0.003 & 22.008$\pm$0.026 & 22.622$\pm$0.026 & -0.466$\pm$0.027 \\
%     % var-ELG22 & [O{\sc ii}]  & 150.074980 & 2.077504 & 24.059$\pm$0.071 & 25.035$\pm$0.025 & 24.561$\pm$0.140 & 25.699$\pm$0.149 & -0.502$\pm$0.157 \\
%     % var-ELG23 & [O{\sc ii}]  & 150.594863 & 2.842712 & 22.773$\pm$0.025 & 23.333$\pm$0.008 & 22.322$\pm$0.028 & 23.344$\pm$0.038 & 0.451$\pm$0.038  \\
%     % var-ELG24 & [O{\sc ii}]  & 150.137929 & 2.513777 & 24.793$\pm$0.104 & 25.158$\pm$0.029 & 24.050$\pm$0.122 & 25.362$\pm$0.120 & 0.743$\pm$0.161  \\
%     % var-ELG25 & [O{\sc ii}]  & 150.126976 & 2.509995 & 24.012$\pm$0.052 & 24.785$\pm$0.019 & 23.533$\pm$0.087 & 24.906$\pm$0.102 & 0.479$\pm$0.101  \\
%     % var-ELG26 & [O{\sc ii}]  & 150.608999 & 2.481510 & 23.801$\pm$0.028 & 24.531$\pm$0.012 & 23.348$\pm$0.077 & 24.392$\pm$0.067 & 0.453$\pm$0.082  \\
%     % var-ELG27 & [O{\sc ii}]  & 150.419160 & 2.049522 & 24.229$\pm$0.026 & 23.774$\pm$0.009 & 22.696$\pm$0.047 & 23.767$\pm$0.048 & 1.533$\pm$0.054  \\ \hline \hline
    
%     var-ELG1  & H$\alpha$   & 150.144353 & 2.228818 & 22.806$\pm$0.023 & 24.005$\pm$0.010 & 23.442$\pm$0.063 & 23.918$\pm$0.055 & -0.637$\pm$0.067 \\
%     var-ELG2  & H$\alpha$   & 149.955213 & 2.607429 & 21.155$\pm$0.005 & 22.268$\pm$0.002 & 21.778$\pm$0.021 & 22.248$\pm$0.021 & -0.623$\pm$0.021 \\
%     var-ELG3  & [O{\sc iii}] & 150.17209  & 2.068556 & 21.225$\pm$0.006 & 22.544$\pm$0.003 & 21.809$\pm$0.021 & 22.535$\pm$0.024 & -0.584$\pm$0.022 \\
%     var-ELG4  & [O{\sc iii}] & 150.161834 & 2.022774 & 20.540$\pm$0.004 & 21.917$\pm$0.002 & 21.057$\pm$0.014 & 21.903$\pm$0.018 & -0.517$\pm$0.015 \\
%     var-ELG5  & [O{\sc iii}] & 150.067333 & 2.473629 & 23.544$\pm$0.028 & 23.623$\pm$0.007 & 22.720$\pm$0.039 & 23.643$\pm$0.042 & 0.825$\pm$0.048  \\
%     var-ELG6  & [O{\sc ii}]  & 149.941078 & 1.963577 & 21.841$\pm$0.010 & 23.000$\pm$0.004 & 22.409$\pm$0.029 & 23.005$\pm$0.031 & -0.567$\pm$0.031 \\
%     var-ELG7  & [O{\sc ii}]  & 149.778466 & 2.762406 & 21.949$\pm$0.013 & 23.092$\pm$0.005 & 22.418$\pm$0.030 & 23.096$\pm$0.034 & -0.469$\pm$0.033 \\
%     var-ELG8  & [O{\sc ii}]  & 150.144187 & 2.750594 & 21.108$\pm$0.006 & 22.731$\pm$0.003 & 21.616$\pm$0.020 & 22.706$\pm$0.027 & -0.508$\pm$0.020 \\
%     var-ELG9  & [O{\sc ii}]  & 149.543688 & 2.553167 & 21.385$\pm$0.007 & 22.633$\pm$0.003 & 21.962$\pm$0.023 & 22.647$\pm$0.026 & -0.577$\pm$0.024 \\
%     var-ELG10 & [O{\sc ii}]  & 150.026968 & 2.116384 & 21.624$\pm$0.007 & 22.792$\pm$0.003 & 22.197$\pm$0.025 & 22.808$\pm$0.028 & -0.573$\pm$0.026 \\
%     var-ELG11 & [O{\sc ii}]  & 150.074999 & 2.077459 & 24.239$\pm$0.071 & 25.189$\pm$0.029 & 24.759$\pm$0.143 & 25.361$\pm$0.117 & -0.520$\pm$0.159 \\
%     var-ELG12 & [O{\sc ii}]  & 150.109818 & 2.286191 & 25.226$\pm$0.114 & 25.318$\pm$0.033 & 24.776$\pm$0.132 & 25.492$\pm$0.131 & 0.450$\pm$0.175  \\
%     var-ELG13 & [O{\sc ii}]  & 150.137929 & 2.513777 & 24.973$\pm$0.104 & 25.319$\pm$0.034 & 24.209$\pm$0.120 & 25.303$\pm$0.115 & 0.765$\pm$0.159  \\
%     var-ELG14 & [O{\sc ii}]  & 150.126957 & 2.510027 & 24.192$\pm$0.052 & 24.759$\pm$0.020 & 23.650$\pm$0.083 & 24.806$\pm$0.094 & 0.543$\pm$0.098  \\ \hline \hline
%     \end{tabular}
%     }
%     \begin{tablenotes}
%     \footnotesize
%     \item Column 1: ID of variable ELGs in this paper; Column 2: emission-line type; Column 3-4: coordinates; Column 5 and 7: corrected NB816 magnitude with HSC and SC as describe in section.~\ref{sec:Variability}; Column 6 and 8: broadband magnitude with HSC and SC; Column 9: variation of NB816 magnitude between HSC- and SC-phase.
%     \end{tablenotes}
%     % \end{threeparttable}
% \end{table*}

% \begin{center}
% \begin{table*}
% \begin{rotatetable*}
% \footnotesize
%     \caption{Physical parameters of variable ELGs}
%     \label{tab:photometry}
%     % \begin{threeparttable}
%     \renewcommand\arraystretch{1.5}
%     % \resizebox{\textwidth}{40mm}{
%     \setlength{\tabcolsep}{0.05cm}{
% \begin{center}
% \begin{tabular}{lccccccccccccccc} \hline \hline
%     \multirow{2}{*}{Var-ID}
%     & \multirow{2}{*}{line}
%     & \multirow{2}{*}{ra} 
%     & \multirow{2}{*}{dec} 
%     & corrected HSC 
%     & HSC i 
%     & corrected SC 
%     & SC i  
%     & variation
%     & X-ray 
%     & MIR  
%     & radio 
%     & \multirow{2}{*}{AGN} 
%     & \multirow{2}{*}{spec-z}  
%     & $\rm SFR_{HSC}$ 
%     & $\rm SFR_{SC}$ 
%     \\
%       &  &  &  & NB816 (mag) & (mag)  & NB816 (mag)  & (mag) & (mag) & AGN  & AGN  & AGN &  &  & ($\rm M_{\odot}\cdot year^{-1}$)& ($\rm M_{\odot}\cdot year^{-1}$)
%     %   & 
%     \\ \hline
%     var-ELG1  & H$\alpha$   & 150.144353 & 2.228818 & 22.806$\pm$0.023 & 24.005$\pm$0.010 & 23.442$\pm$0.063 & 23.918$\pm$0.055 & -0.637$\pm$0.067 & 0 & 0 & 0 & 0 & 0.236 & 0.18$^a$/0.12$^b$  & 0.10$^a$/0.07$^b$  \\
%     var-ELG2  & H$\alpha$   & 149.955213 & 2.607429 & 21.155$\pm$0.005 & 22.268$\pm$0.002 & 21.778$\pm$0.021 & 22.248$\pm$0.021 & -0.623$\pm$0.021 & 0 & 0 & 0 & 0 & 0.237 & 0.86$^a$/0.58$^b$  & 0.51$^a$/0.34$^b$  \\
%     var-ELG3  & [O{\sc iii}] & 150.17209  & 2.068556 & 21.225$\pm$0.006 & 22.544$\pm$0.003 & 21.809$\pm$0.021 & 22.535$\pm$0.024 & -0.584$\pm$0.022 & 0 & 0 & 0 & 0 & 0.62  & 6.06$^c$  & 3.78$^c$  \\
%     var-ELG4  & [O{\sc iii}] & 150.161834 & 2.022774 & 20.540$\pm$0.004 & 21.917$\pm$0.002 & 21.057$\pm$0.014 & 21.903$\pm$0.018 & -0.517$\pm$0.015 & 0 & 0 & 0 & 0 & 0.62  & 11.39$^c$ & 7.56$^c$  \\
%     var-ELG5  & [O{\sc iii}] & 150.067333 & 2.473629 & 23.544$\pm$0.028 & 23.623$\pm$0.007 & 22.720$\pm$0.039 & 23.643$\pm$0.042 & 0.825$\pm$0.048  & 0 & 0 & 0 & 0 & 0.636 & 0.76$^c$  & 1.74$^c$  \\
%     var-ELG6  & [O{\sc ii}]  & 149.941078 & 1.963577 & 21.841$\pm$0.010 & 23.000$\pm$0.004 & 22.409$\pm$0.029 & 23.005$\pm$0.031 & -0.567$\pm$0.031 & 0 & 0 & 0 & 0 & 1.175 & 20.39$^d$ & 12.93$^d$ \\
%     var-ELG7  & [O{\sc ii}]  & 149.778466 & 2.762406 & 21.949$\pm$0.013 & 23.092$\pm$0.005 & 22.418$\pm$0.030 & 23.096$\pm$0.034 & -0.469$\pm$0.033 & 0 & 0 & 0 & 0 & 1.175 & 18.47$^d$ & 12.82$^d$ \\
%     var-ELG8  & [O{\sc ii}]  & 150.144187 & 2.750594 & 21.108$\pm$0.006 & 22.731$\pm$0.003 & 21.616$\pm$0.020 & 22.706$\pm$0.027 & -0.508$\pm$0.020 & 0 & 0 & 0 & 0 & 1.175 & 40.07$^d$ & 26.82$^d$ \\
%     var-ELG9  & [O{\sc ii}]  & 149.543688 & 2.553167 & 21.385$\pm$0.007 & 22.633$\pm$0.003 & 21.962$\pm$0.023 & 22.647$\pm$0.026 & -0.577$\pm$0.024 & 0 & 0 & 0 & 0 & 1.175 & 31.04$^d$ & 19.50$^d$ \\
%     var-ELG10 & [O{\sc ii}]  & 150.026968 & 2.116384 & 21.624$\pm$0.007 & 22.792$\pm$0.003 & 22.197$\pm$0.025 & 22.808$\pm$0.028 & -0.573$\pm$0.026 & 0 & 0 & 0 & 0 & 1.176 & 24.98$^d$ & 15.75$^d$ \\
%     var-ELG11 & [O{\sc ii}]  & 150.074999 & 2.077459 & 24.239$\pm$0.071 & 25.189$\pm$0.029 & 24.759$\pm$0.143 & 25.361$\pm$0.117 & -0.520$\pm$0.159 & 0 & 0 & 0 & 0 & 1.177 & 2.25$^d$  & 1.49$^d$  \\
%     var-ELG12 & [O{\sc ii}]  & 150.109818 & 2.286191 & 25.226$\pm$0.114 & 25.318$\pm$0.033 & 24.776$\pm$0.132 & 25.492$\pm$0.131 & 0.450$\pm$0.175  & 0 & 0 & 0 & 0 & 1.187 & 0.93$^d$  & 1.50$^d$  \\
%     var-ELG13 & [O{\sc ii}]  & 150.137929 & 2.513777 & 24.973$\pm$0.104 & 25.319$\pm$0.034 & 24.209$\pm$0.120 & 25.303$\pm$0.115 & 0.765$\pm$0.159  & 0 & 0 & 0 & 0 & 1.197 & 1.19$^d$  & 2.58$^d$  \\
%     var-ELG14 & [O{\sc ii}]  & 150.126957 & 2.510027 & 24.192$\pm$0.052 & 24.759$\pm$0.020 & 23.650$\pm$0.083 & 24.806$\pm$0.094 & 0.543$\pm$0.098  & 0 & 0 & 0 & 0 & 1.198 & 2.45$^d$  & 4.32$^d$  \\ \hline \hline
%     \end{tabular}
%     \tablecomments{Column 1: ID of variable ELGs in this paper; Column 2: emission-line type; Column 3-4: coordinates; Column 5 and 7: corrected NB816 magnitude with HSC and SC as describe in section.~\ref{sec:Variability}; Column 6 and 8: broadband magnitude with HSC and SC; Column 9: variation of NB816 magnitude between HSC- and SC-phase. Column 10-11: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite; Column 12: radio selected AGN from~\citet{Delvecchio2017}; Column 13: total number of AGN via above three methods; Column 14: spectroscopic redshift; Column 15-16: SFRs of variable ELGs calculated by emission-line indicator in HSC-phase and SC-phase, as described in section~\ref{sec:SFR}. $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; $^c$ follows~\citet{Zhuang2019}; $^d$ follows~\citet{Villa2021}.}
    
% % \begin{tablenotes}
% %     \footnotesize
% %     \item Column 1: ID of variable ELGs in this paper; Column 2: emission-line type; Column 3-4: coordinates; Column 5 and 7: corrected NB816 magnitude with HSC and SC as describe in section.~\ref{sec:Variability}; Column 6 and 8: broadband magnitude with HSC and SC; Column 9: variation of NB816 magnitude between HSC- and SC-phase. Column 10-11: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite; Column 12: radio selected AGN from~\citet{Delvecchio2017}; Column 13: total number of AGN via above three methods; Column 14: spectroscopic redshift; Column 15-16: SFRs of variable ELGs calculated by emission-line indicator in HSC-phase and SC-phase, as described in section~\ref{sec:SFR}. $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; $^c$ follows~\citet{Zhuang2019}; $^d$ follows~\citet{Villa2021}.
% % \end{tablenotes}

% \end{center}
% }
% \end{rotatetable*}
% \end{table*}
% \end{center}



\begin{sidewaystable*}
% \begin{table*}
    \centering
    \footnotesize
    \caption{\revise{Physical Parameters of Variable ELGs}}
    \label{tab:photometry}
    \renewcommand\arraystretch{1.2}
    % \resizebox{\textwidth}{40mm}{
    \setlength{\tabcolsep}{0.05cm}{
    \begin{tabular}{lccccccccccccccc} \hline \hline
    \multirow{2}{*}{Var-ID}
    & \multirow{2}{*}{line}
    & \multirow{2}{*}{ra} 
    & \multirow{2}{*}{dec} 
    & corrected HSC 
    & HSC i 
    & corrected SC 
    & SC i  
    & $\rm\Delta m_{NB816}$
    & X-ray 
    & MIR  
    & radio 
    & \multirow{2}{*}{AGN} 
    & \multirow{2}{*}{spec-z}  
    & $\rm SFR_{HSC}^1$ 
    & $\rm SFR_{SC}^1$ 
    \\
      &  &  &  & NB816 (mag) & (mag)  & NB816 (mag)  & (mag) & (mag) & AGN  & AGN  & AGN &  &  & ($M_{\odot}\,\rm yr^{-1}$)& ($M_{\odot}\,\rm yr^{-1}$)
    %   & 
    \\ \hline
    var-ELG1 & [O{\sc iii}] & 150.547364 & 2.804791 & 21.799$\pm$0.020 & 21.949$\pm$0.006 & 21.421$\pm$0.027 & 21.941$\pm$0.034 & 0.378$\pm$0.033 & 0 & 0 & 0 & 0 & 0.623 & 0.14 & 1.71  \\
    var-ELG2 & [O{\sc iii}] & 150.268059 & 2.775813 & 21.282$\pm$0.010 & 21.677$\pm$0.004 & 21.008$\pm$0.022 & 21.659$\pm$0.030 & 0.275$\pm$0.024 & 0 & 0 & 0 & 0 & 0.623 & 1.46 & 3.18  \\
    var-ELG3 & [O{\sc iii}] & 150.067333 & 2.473629 & 23.544$\pm$0.071 & 23.623$\pm$0.023 & 22.720$\pm$0.067 & 23.643$\pm$0.080 & 0.825$\pm$0.097 & 0 & 0 & 0 & 0 & 0.636 & -0.03 & 0.95  \\
    var-ELG4 & [O{\sc iii}] & 150.681233 & 2.763416 & 20.968$\pm$0.010 & 21.610$\pm$0.005 & 20.743$\pm$0.022 & 21.608$\pm$0.031 & 0.225$\pm$0.024 & 0 & 0 & 0 & 0 & 0.636 & 3.46 & 5.54 \\
    var-ELG5 & [O{\sc iii}] & 149.936369 & 1.990318 & 21.827$\pm$0.016 & 22.504$\pm$0.008 & 21.582$\pm$0.036 & 22.511$\pm$0.045 & 0.245$\pm$0.039 & 0 & 0 & 0 & 0 & 0.637 & 1.65 & 2.72  \\ 
    \hline 
    \end{tabular}
    }
    %  \tablecomments{Column 1: ID of variable ELGs in this paper; Column 2: emission-line type; Column 3-4: coordinates; Column 5 and 7: corrected NB816 magnitude with HSC and SC as describe in section.~\ref{sec:Variability}; Column 6 and 8: broadband magnitude with HSC and SC; Column 9: variation of NB816 magnitude between HSC- and SC-phase. Column 10-11: X-ray and MIR selected AGN. 1 represented that the object was confirmed as AGN, 0 is at opposite; Column 12: radio selected AGN from~\citet{Delvecchio2017}; Column 13: total number of AGN via above three methods; Column 14: spectroscopic redshift; Column 15-16: SFRs of variable ELGs calculated by emission-line indicator in HSC-phase and SC-phase, as described in section~\ref{sec:SFR}. $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; $^c$ follows~\citet{Zhuang2019}; $^d$ follows~\citet{Villa2021}.}
    \begin{tablenotes}
    \footnotesize
    \item Column 1: ID of variable ELGs in this paper; Column 2: emission-line type; Column 3-4: coordinates (equatorial); Column 5 and 7: corrected NB816 magnitude with HSC and SC as describe in section.~\ref{sec:Variability}; Column 6 and 8: broadband magnitude with HSC and SC; Column 9: NB816-magnitude differences between NB816 observations with HSC and SC. Column 10-12: X-ray, MIR and radio selected AGN. 0 means non-detection; Column 13: total number of AGN via above three methods; Column 14: spectroscopic redshift; Column 15-16: two-epoch SFRs of variable ELGs calculated by SFR-emission-line indicators. 
    % $^a$ follows~\citet{Kennicutt1998}; $^b$ follows~\citet{Kennicutt2012}; 
    $^1$ SFR([O{\sc iii}]) following~\citet{Zhuang2019}.
    % ; $^b$ SFR([O{\sc ii}]) following~\citet{Villa2021}.
    \end{tablenotes}
% \end{table*}
\end{sidewaystable*}



==> variable ELG/table/table_sextractor_para.tex <==
\begin{table}
% \centering
% \footnotesize
\centering
\caption{SExtractor Parameters Used in the Duel-mode}
\label{tab:sext_para}
% \resizebox{\textwidth}{15mm}{
\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{llr} 
\hline \hline
parameter         &  &value                 \\ \hline
--------------------&  Extraction &--------------------\\
DETECT\_TYPE      &  &CCD                   \\
DETECT\_MINAREA   &  &5                     \\
DETECT\_MAXAREA   &  &100000                \\
DETECT\_THRESH    &  &0.6 (in sigma)                   \\
ANALYSIS\_THRESH  &  &0.6 (in sigma)                   \\
FILTER            &  &Y                     \\
FILTER\_NAME      &  &gauss\_2.5\_5x5.conv  \\
DEBLEND\_NTHRESH  &  &64                    \\
DEBLEND\_MINCONT  &  &0.00001              \\
CLEAN             &  &Y                     \\
CLEAN\_PARAM      &  &1                     \\
--------------------& Photometry &--------------------\\
PHOT\_APERTURES   &  &17.65,2.94,11.76,35        \\
PHOT\_AUTOPARAMS  &  &2.5, 3.5              \\
PHOT\_PETROPARAMS &  &2.0, 3.5              \\
PHOT\_AUTOAPERS   &  &0.0, 0.0              \\
PHOT\_FLUXFRAC    &  &0.2,0.5,0.8           \\
SATUR\_LEVEL      &  &50000                 \\
SATUR\_KEY        &  &SATURATE              \\
MAG\_ZEROPOINT    & SC NB816    & 31.07  \\
                  & SC i        & 31.17  \\
                  & HSC NB816   & 26.98  \\
                  & HSC i       & 27.02  \\
MAG\_GAMMA        &  &4                     \\
GAIN              &  &0                     \\
GAIN\_KEY         &  &GAIN                  \\
PIXEL\_SCALE      &  &0.17                  \\
SEEING\_FWHM      & SC NB816    & 0.95  \\
                  & SC i        & 0.95  \\
                  & HSC NB816   & 0.73  \\
                  & HSC i       & 0.66  \\
--------------------& Background &--------------------\\
BACK\_TYP         &  &AUTO                  \\
BACK\_VALUE       &  &0                     \\
BACK\_SIZE        &  &128                   \\
BACK\_FILTERSIZE  &  &3                     \\
BACKPHOTO\_TYPE   &  &LOCAL                 \\
BACKPHOTO\_THICK  &  &30                    \\
% ------& Star/Galaxy Separation &-------\\

\hline 
\end{tabular}
}
\end{table}
